Simulation Over One-counter Nets is PSPACE-Complete

One-counter nets (OCN) are Petri nets with exactly one unbounded place. They are equivalent to a subclass of one-counter automata with just a weak test for zero. Unlike many other semantic equivalences, strong and weak simulation preorder are decidable for OCN, but the computational complexity was an open problem. We show that both strong and weak simulation preorder on OCN are PSPACE-complete.

==> pictures/behind.tex <==
\begin{tikzpicture}[scale=0.65]
  \path[draw,use as bounding box](-4,-2.4) rectangle (7,3.4);
    \coordinate(0) at (0,0);
    \draw (0) edge[dotted] (-2,-2);
    \draw[->,thick](0) -- (3,3) node[right] {$(\rho,\rho')$};
    \draw[->](0) -- (2,0.5) node[right] {$(\alpha,\alpha')$};
    \draw[->](0) -- (1,-1.5) node[right] {$(\beta,\beta')$};
    %\draw[->](0) -- (1,2) node[left] {$(\gamma,\gamma')$};
    \draw[->](0) -- (-1,1) node[left] {$(\delta,\delta')$};
\end{tikzpicture}



==> pictures/outcome.tex <==
\begin{tikzpicture}[scale=0.65]
  \path[draw,use as bounding box](-4,-2.4) rectangle (6,3.4);
  \def\w{4cm}
  \def\SpC{red!50}
  \def\DupC{green!50}
  \def\ContC{yellow!70}
  \coordinate (RHO) at (3,3);
  \coordinate (RS) at (-2,-2);
  \coordinate (TL) at (-\w,\w);
  \coordinate (T) at (0,\w);
  \coordinate (B) at (0,-\w);
  \coordinate (R) at (\w,0);
  \coordinate (L) at (-\w,0);
  \coordinate (TR) at (\w,\w);
  \coordinate (BL) at (-\w,-\w);
  \coordinate (BR) at (\w,-\w);

  %\fill[blue!20!] (TR) rectangle (BL);
  %\fill[red!20] (0,0) -- (BL) -- (TL) -- (0,\w)-- cycle;
  %\fill[green!10] (0,0) -- (TR) -- (BR) -- (BL)-- cycle;

  % DUPLICATOR WINS %%%%%%%%%%%%%%%%%%%%%%%%%
  % draw and clip coloured circle
  \begin{scope}
    \path[clip] (RHO) -- (TL) -- (BL);
    \fill[\DupC, path fading=fade out] (0,0) circle (2cm);
  \end{scope}
  % compute label position
  \path[bend left] ($(0,0)!1cm!(RS)$) to coordinate [midway] (mid) ($(0,0)!1cm!(RHO)$); % Get half angle
  \coordinate (labelpos) at ($(0,0)!3cm!(mid)$);
  % place label
  \node[align=center] at (labelpos) {\V\\wins};
  
  % GAME CONTINUES %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % draw and clip coloured circle
  \begin{scope}
    \path[clip] (RHO) -- (TR) -- (R) -- (0,0);
    \fill[\ContC, path fading=fade out] (0,0) circle (4cm);
  \end{scope}
  % compute label pos
  \path ($(0,0)!1cm!(RHO)$) to coordinate [midway] (mid) ($(0,0)!1cm!(R)$); % Get half angle
  \coordinate (labelpos) at ($(0,0)!4cm!(mid)$);
  % place label
  \node[align=center] at (labelpos) {Game\\continues};
  
  % SPOILER WINS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{scope}
      \path[clip] (0,0) -- (R) -- (BR) -- (RS);
    \fill[red, path fading=fade out] (0,0) circle (1.5cm);
  \end{scope}
  % compute label pos
  \path ($(0,0)!1cm!(RS)$) to coordinate [midway] (mid) ($(0,0)!1cm!(R)$);
  \coordinate (labelpos) at ($(0,0)!2cm!(mid)$);
  % place label
  \node at (labelpos) {\R\ wins};
  
  \draw[dash pattern=on5pt off3pt] (\w,0) -- (0,0);
  \draw[dash pattern=on2pt off2pt] (0,0) -- (RS);
  %\draw[thick,->] (0,0) -- (RHO);
  %\node[right of=RHO] {$(\rho,\rho')$};
  \draw[->,thick](0) -- (RHO) node[right] {$(\rho,\rho')$};
    
  
  \coordinate(0) at (0,0);
    \draw[->](0) -- (2,0.5);
    \draw[->](0) -- (1,-1.5);
    \draw[->](0) -- (-1,1);
\end{tikzpicture}



==> pictures/vert_belt.tex <==
  \def\c{1}
  \def\RX{5}
  \def\RY{2.5}
  \def\xmax{8}
  \def\ymax{6.5}
  \def\width{8.5}
  \def\height{6}
  \def\xaxispoints{0, 0.5, 1, 1.5, 2, 2.5, 3, 3.5, 4}
  \def\yaxispoints{0, 0.5, 1, 1.5, 2, 2.5, 3, 3.5, 4}
  \def\offset{0}
  \begin{tikzpicture}[scale=0.7]
    \tikzstyle{every node}=[font=\small]
    \coordinate (rhorho') at (0,\RY);
    % -------------------------
    % Grid
    \draw[step=0.25,blue!5!white, very thin] (3,0) grid (\width,\height);
    \draw[decorate,decoration={brace,raise=0pt, amplitude=10pt}, thick] (3,0)--(3,3.5);      
    \node (no1) at (1.5,1.7) {aperiodic};
    \draw[decorate,decoration={brace,raise=0pt, amplitude=10pt}, thick] (3,3.5)--(3,6);      
    \node (no2) at (1.5,4.7) {periodic};
    
    \draw[decorate,decoration={brace,raise=0pt,mirror , amplitude=10pt}, thick] (3,0)--(6,0);      
    \node (no3) at (5,-1) {\begin{minipage}[adjusting]{3cm}
    bound for the \\ width of a belt
    \end{minipage}
    };

    
    % -------------------------
    % Axis
    \draw[name path=yaxis, ->] (3,0) -- ($(3,\height)$) node[black,above] {\V\ $n'$};
    \draw[name path=xaxis, ->] (3,0) -- ($(\width,0)$) node[black,right] {\R\ $n$};

    % -------------------------
%    % define points above and 0C
%    \coordinate (above) at ($(rhorho')+(-\c,\c)$);
%    \path[name path=upper] (above) -- +(-\RX, -\RY);
%    \path [name intersections={of=upper and yaxis,by=0C}];

%    % -------------------------
%    % define points below and C0
%    \coordinate (below) at ($(rhorho')+(\c,-\c)$);
%    \path[name path=lower] (below) -- +(-\RX, -\RY);
%    \path[name intersections={of=lower and xaxis,by=C0}];

    % -------------------------
    % draw the rest within the rectangle (0,0) to (\xmax,\ymax)
    \begin{scope}
      \path[clip, name path=border] (3,0) -- (3,\ymax) -- (\xmax,\ymax) -- (\xmax,0);
      \path[name path=outerborder] (3,\ymax) -- (\xmax,\ymax) -- (\xmax,0);  % used to calculate intersections
      % -------------------------
      % (rho,rho') and continuation
      \draw[->] (6,0) -- ($(6,0)+.5*(rhorho')$) node[right]{$(\rho,\rho')$};
      \draw[densely dashed, segment length=20pt] ($(6,0)+.6*(rhorho')$) -- ($(6,0)+2*(rhorho')$);
      
      \draw[-] (3,.25) -- ($(3.25,.5)$) node[right]{$$};
      \draw[-] (3.25,.5) -- ($(4,.5)$) node[right]{$$};
      \draw[-] (4,.5) -- ($(4.25,1)$) node[right]{$$};
      \draw[-] (4.25,1) -- ($(4.5,1.25)$) node[right]{$$};
      \draw[-] (4.5,1.25) -- ($(4.75,2)$) node[right]{$$};
      \draw[-] (4.75,2) -- ($(5,3.5)$) node[right]{$$};
      \draw[-] (5,3.5) -- ($(5.5,3.5)$) node[right]{$$};
      \draw[-] (5.5,3.5) -- ($(5.5,6)$) node[right]{$$};

      % -------------------------
%      % upper c-square
%      \draw[dotted] (rhorho') edge node[below] {c} ($(rhorho')+(-\c,0)$);
%      \draw[dotted] ($(rhorho')+(-\c,0)$) edge node[left] {c} ($(rhorho')+(-\c,\c)$);
%      \draw[dotted] ($(rhorho')+(-\c,\c)$) -- ($(rhorho')+(0,\c)$);
%      \draw[dotted] ($(rhorho')+(0,\c)$) -- (rhorho');

      % -------------------------
      % lower c-square
%      \draw[dotted] (rhorho')
%                    -- ($(rhorho')+(\c,0)$)
%                    -- (below)
%                    -- ($(rhorho')+(0,-\c)$)
%                    -- cycle;

      % -------------------------
      % belt lines
%     \draw[name path=lower] (C0) -- ($(C0)+50*(rhorho')$);  % lower line
    %  \draw[name path=upper] (0C) -- ($(0C)+20*(rhorho')$);  % upper line
      
      % -------------------------
      % label upper segment
%      \path[name intersections={of=upper and outerborder,by=upperEnd}];
%      \coordinate (midabove) at ($(upperEnd)!.5!(0,\ymax)$);
     \node (yes) at (5,4) {$\preceq$};
      
      % -------------------------
      % label lower segment
    %  \path[name intersections={of=lower and outerborder,by=lowerEnd}];
     % \coordinate (midbelow) at ($(lowerEnd)!.5!(\xmax,0)$);
      \node (no) at (7,2) {$\not\preceq$};
      
      
      
      
    \end{scope}
  \end{tikzpicture}

